Consistency Regularization with High-dimensional Non-adversarial Source-guided Perturbation for Unsupervised Domain Adaptation in Segmentation

Unsupervised domain adaptation for semantic segmentation has been intensively studied due to the low cost of the pixel-level annotation for synthetic data. The most common approaches try to generate images or features mimicking the distribution in the target domain while preserving the semantic contents in the source domain so that a model can be trained with annotations from the latter. However, such methods highly rely on an image translator or feature extractor trained in an elaborated mechanism including adversarial training, which brings in extra complexity and instability in the adaptation process. Furthermore, these methods mainly focus on taking advantage of the labeled source dataset, leaving the unlabeled target dataset not fully utilized. In this paper, we propose a bidirectional style-induced domain adaptation method, called BiSIDA, that employs consistency regularization to efficiently exploit information from the unlabeled target domain dataset, requiring only a simple neural style transfer model. BiSIDA aligns domains by not only transferring source images into the style of target images but also transferring target images into the style of source images to perform high-dimensional perturbation on the unlabeled target images, which is crucial to the success in applying consistency regularization in segmentation tasks. Extensive experiments show that our BiSIDA achieves new state-of-the-art on two commonly-used synthetic-to-real domain adaptation benchmarks: GTA5-to-CityScapes and SYNTHIA-to-CityScapes.

==> figures/tex/alpha.tex <==
\begin{figure*}[t]
\centering
\captionsetup[subfigure]{labelformat=empty}
   \subfloat[ Source image \label{fig:PKR}]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/content.png}}
\hspace{2em}
   \subfloat[ $\alpha=0$ \label{fig:PKT} ]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/alpha_0.png}}
\hspace{0.5em}
   \subfloat[ $\alpha=0.2$ \label{fig:tie5}]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/alpha_0_2.png}}
\hspace{0.5em}
   \subfloat[ $\alpha=0.4$ \label{fig:tie5}]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/alpha_0_4.png}}
\vspace{1.3em}
\\ [-5ex]
      \subfloat[ Target image \label{fig:PKR}]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/style.png}}
\hspace{2em}
   \subfloat[ $\alpha=0.6$ \label{fig:PKT} ]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/alpha_0_6.png}}
\hspace{0.5em}
   \subfloat[ $\alpha=0.8$ \label{fig:tie5}]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/alpha_0_8.png}}
\hspace{0.5em}
   \subfloat[ $\alpha=1$ \label{fig:tie5}]{%
      \includegraphics[width=4cm, height=2cm]{figures/fig/alpha/alpha_1.png}}
      \\[-4ex]
      
\vspace{0.5cm}
\caption{\small Output images of our continuous style-guided image generator with different content-style trade-off parameter $\alpha$.}
    \label{fig:sample_images}
\end{figure*}

==> sections/abstract.tex <==
\begin{abstract}
Unsupervised domain adaptation for semantic segmentation has been intensively studied due to the low-cost of the pixel-level annotation for synthetic data. Most current approaches [performing pixel-level alignment] essentially rely on constructing an elaborated image translator (or feature extractor) that generates images (or features) mimicking the distribution of target domain images while keeping the semantic contents of the source domain so that a segmentation model will be trained on the source dataset with target-domain-like images with pixel-level annotation, leaving the unlabeled target images not fully utilized. In this paper, we propose a [bidirectional consistency regularization] method that employs consistency regularization to efficiently exploit information from the unlabeled target domain dataset, requiring only a simple neural style transfer model. Domains are aligned by not only transferring source images into the style of target images but also transferring target images into the style of source images to guide the training on the unlabeled target images. In comparison with other methods, several experiments reveal that our approach achieves the state-of-the-art performance.
\end{abstract}

==> sections/acknowledgement.tex <==
%section{ Acknowledgements}
% Margrit's grant
%We acknowledge partial support of this work by the ONR MURI Program, N00014-19-1-2571 associated with AUSMURIB000001.

==> sections/conclusion.tex <==
\section{Conclusion}
This is the best UDA segmentation model!!

==> sections/experiments.tex <==
\input{tables/gta2cityscape}
\input{tables/synthia2cityscape}

\section{Experiments}

The section describes the experiments with our method OUR-NAME on two synthetic-to-real segmentation benchmark datasets, ablation studies, and comparisons with other methods.

% Margrit commented this out because it is too detailed for the intro of the Experiment section and will be described anyway:
%Our method is evaluated on two competitive synthetic-to-real segmentation benchmarks, namely GTA V~\cite{RichterViRoKo16} - Cityscapes~\cite{CordtsOmRaReEnBeFrRoSc16} and Synthia~\cite{RosSeMaVaLo16} - Cityscapes~\cite{C}, using two segmentation models with different backbones, VGG16~\cite{SimonyanZi14} and ResNet101~\cite{HeZhReSu16}. 


\subsection{Datasets}

%Margrit to all: Almost have a space between a word and the citation
The Cityscapes dataset~\cite{CordtsOmRaReEnBeFrRoSc16} consists of real-world images of street scenes in multiple cities in Germany. Each image has a spatial resolution of 2048$\times$1024 pixels. The training dataset includes 2,975 images, the validation set 500 images, and the test set 1,525 images. Pixel-level annotations among 19 semantic categories are provided for the images in the training and validation set.  In our experiments, we used the 500 images in the validation set as our test set.  

The  GTA V dataset~\cite{RichterViRoKo16} includes 24,966 synthetic images with a resolution of 1914$\times$1052 pixels, which were obtained from the video game GTA V along with pixel-level annotations that share all 19 common categories with the Cityscapes dataset.
From the Synthia dataset~\cite{RosSeMaVaLo16}, we use the SYNTHIA-RAND-CITYSCAPES subset, which contains 9,400 rendered images of size 1280$\times$760 and shares 16 common categories with the Cityscapes dataset.

\subsection{Experiments with Backbone Networks}
 
 To evaluate our method, we experimented with the architecture of our segmentation network.  We adopted the Deeplabv2 model~\cite{} with a ResNet101 model~\cite{HeZhReSu16} as our backbone network and, alternatively, FCN-8s~\cite{ShelhamerLoDa15} with a VGG16~\cite{SimonyanZi15} as the backbone network. Both backbone networks were pre-trained with the ImageNet data~\cite{KrizhevskySuHi12}.



\subsection{Training Protocol}
GPU; Optimizer; learning rate adjuster, weight decay


\subsection{Ablation Studies}


\subsection{Results and Comparisons with Other Methods}

Our method NAME performed accurately .... details... (Table~\ref{table:main-results}).

Better than state-of-the-art models XYZ by .... percent points (pp).   


\subsection{Discussion}

What was revealed by experiments?
Why better? 

What are still limitations?

==> sections/introduction.tex <==
\section{Introduction}
% Margrit recommends:
% Please don't use a separate file for all the tables, figures, sections (as in the ECCV 2020 paper).
% It's much easier&faster to work with a single file.
% Especially searching is difficult with a multi-file structure...


% Margrit recommends:
%Describe the UDA problem.\\
%Introduce current methods and their limitations.\\
%Introduce our method and its advantages, especially how it cope with the limitation and problem mentioned above.\\
%%%%%%%
%%%%%%%
Deep learning methods for semantic segmentation~\cite{ShelhamerLoDa15}, the problem of dividing the pixels in an image into mutually exclusive and collectively exhaustive sets of class-labeled regions,  have gained increasing attention due to their surprising performance and indispensable role in various image analysis tasks, including autonomous driving and computed-aided medical diagnosis.  Research progress, however, is hindered by the difficulty of creating large training datasets with accurate pixel-level annotations of these regions.  Manual pixel-level annotation of an image in the Cityscapes dataset, for example, and its quality control typically require more than 1.5 hours~\cite{Cordts2016Cityscapes}, an expensive and time-consuming process. As a consequence, the use of synthetic datasets has become popular because pixel-level ground truth annotations can be generated along with the images. Unfortunately, when deep models that were trained on synthetic data are used to segment real-world images, their performance is typically limited due to the domain gap between the training and testing data.  Domain adaptation methods seek to bridge the gap between the source domain training data and the target domain testing data.  We here focus on unsupervised domain adaptation (UDA), the problem of adapting a model that was trained with a labeled source domain dataset, by using an unlabeled target domain dataset and optimizing its performance on the target domain.
%%%%%%%
%%%%%%%
% With the unprecedented development in the area of deep learning, semantic segmentation~\cite{ShelhamerLoDa15} has gained increasing attention due to its surprising performance and indispensable role in various application scenarios including autonomous driving and medical imaging. However, the rapid progression is limited by the difficulty of acquiring a large dataset with pixel-level annotation. According to ~\cite{CordtsOmRaReEnBeFrRoSc16}, fine pixel-level annotation and quality control require more than 1.5 hours on average for a single image, which is expensive and time-consuming. As a consequence, synthetic datasets become a popular option since its corresponding pixel-wise annotation could be generated along with images. Unfortunately, a domain gap between a synthetic image dataset and a real-world image dataset constantly exists, bringing in the necessity of performing unsupervised domain adaptation(UDA) which adapt a model trained on a labeled source domain dataset with an unlabeled target domain dataset and optimize its performance on the latter.

To align the domain of a labeled source dataset to the domain of a target dataset on a pixel-level or feature-level basis,
existing segmentation methods typically use adversarial training~\cite{GoodfellowPoMiXuWaOzCoBe14}, supervised by the loss with the annotation of the source domain dataset and agnostic to the unlabeled target dataset. 
% Margrit writes: The intro is too wordy and needs to come to our own work sooner and what its differences are.
%Existing methods typically focus on aligning the domain of a labeled source dataset to a target dataset on pixel-level or feature-level using adversarial training~\cite{GoodfellowPoMiXuWaOzCoBe14} so a supervised loss can be computed with the annotation of the source domain dataset to guide the training a segmentation model. 
% Margrit:  This next section is too long to get to the point. Others (Choi, Xu et al) already work on semi-supervised...
In spite of the closer domain gap, the employment of adversarial training brings in extra complexity and instability to the training process. What is worse is that the utilization of the unlabeled target dataset is often overlooked when these methods pay major attention on the domain adaptation problem of UDA. In this work, we argue that semi-supervised learning is an effective approach to learn from an unlabeled dataset and should be taken into consideration.
Some existing methods indeed employ classic semi-supervised learning approaches, including entropy minimization~\cite{VuJaBuCoPe19} and pseudo-labeling~\cite{LiYuVa19,YangSo20,ZouYuKuWw18}, but these approaches to use the unlabeled data either only play an auxiliary role in the training process or fail to boost the performance significantly, revealing the difficulty of leveraging classical semi-supervised learning methods for the task of segmentation. Inspired by progress in consistency regularization methods, self-ensemble models that utilize pseudo-labeling and consistency regularization to learn from the unlabeled dataset have been proposed~\cite{ChoiKiKi19,XuDuZhZhWaZh19}. Nevertheless, as ~\cite{FrenchAiLaMaFi2019} has indicated that perturbations for consistency regularization in semi-supervised semantic segmentation require semantic constraint, these methods augment target samples with just low-dimensional transformation such as adding Gaussian Noise or performing color jitters, which limit the potentials of consistency learning on segmentation tasks.

%ADD THE LIMITATIONS of Choi et al and Xu et al. IS IT JUST ACCURACY?  OR A METHODOLOGICAL LIMITATION?  WHY IS OUR WORK BETTER THAN THEIRS?
%SET THE STAGE FOR OUR WORK.  WHAT IS DIFFERENT and NEW ABOUT OUR APPROACH?

%THE NEXT SECTION IS JUST ABOUT WHAT WE DO NOT WHICH LIMITATION/DIFFICULTY WE OVERCOME.  WHAT WE DO CAN BE DESCRIBED IN DETAIL LATER.  SO HERE JUST THE GIST IS IMPORTANT. 
%Motivated by recent progress in semi-supervised learning area, 
In this paper, we propose a novel consistency regularization method that optimizes a segmentation model through a supervised and an unsupervised loss. The problem of domain adaptation is tackled by a simple yet effective pre-trained style transfer network in both the supervised and unsupervised phases while a consistency learning module addresses the utilization of the unlabeled target domain dataset. For the supervised loss, we adopt the style transfer network to generate source domain images with target domain style and corresponding pixel-level annotation to train a segmentation model and minimize the domain gap. For the unsupervised loss, the style transfer network will be used to augment target images with semantic constraint by transferring the style of the target domain images to a source-domain-like style that the segmentation model is more familiar with and therefore can interpret more accurately. The transferred images are passed through an self-ensemble of trained segmentation models
% (MARGRIT ASKS: ensemble=collection -- do you mean "ensemble of trained segmentation models")
to produce high-quality pseudo labels, which guide the training of the target domain images with fundamental augmentation as in ~\cite{ChoiKiKi19} on a segmentation model.
%MARGRIT: "weak augmentation" is not clear here.
In conclusion, our contribution includes:
\begin{enumerate}
  \item
    We propose a [source-transferred] perturbation method on target images for consistency regularization specialized in unsupervised domain adaptation for semantic segmentation;
  \item
    We combine a [target-transferred] supervised learning with a [source-transferred] unsupervised learning and show that both process can boost the performance of each other without requiring an complicated/elaborated image translator;
  \item
    Several experiments on different datasets and network architectures showing that our method achieves STATE-OF-THE-ART performance.
\end{enumerate}

==> sections/methods.tex <==
\section{Method}

In this paper, we propose a framework that performs domain adaptation and semi-supervise learning using self-ensembling~\cite{TarvainenVa17} and consistency regularization with novel perturbation methods specialized for semantic segmentation task. The training process includes a target-guided supervised learning phase and an source-guided unsupervised learning phase. A simple yet effective image translator that synthesizes images with different styles is pretrained and will be applied in both the supervised and unsupervised phase. For the supervised phase, a cross entropy loss will be computed by a synthesized image and the pixel-level annotation to merge the domain gap. For the unsupervised phase, we average the score map of a series of target domain images transferred with the style of source domain images through a teacher model and produce a pseudo-label which guides the training of the same target image with only fundamental color space augmentation on the student network through a cross entropy loss.

% Important: will be good if we can show that our framework can work well without self-ensembling.

Formally, Under UDA settings, the dataset from the source domain $\mathcal{S}$ includes images denoted by ${X^\mathcal{S}}$ with its corresponding pixel-level annotation denoted by ${Y^\mathcal{S}}$, while the dataset from the target domain $\mathcal{T}$ contains images represented by $X^\mathcal{T}$ without annotation. Formally, we need to optimize a segmentation model using $N^\mathcal{S}$ pairs of source data $\{x_i^\mathcal{S}, y_i^\mathcal{S}\}$ from the source dataset and $N^\mathcal{T}$ target images $\{x_i^\mathcal{T}\}$ on $\mathcal{C}$ common categories. 

To stabilize the generation of pseudo-label, we employ self-ensembling~\cite{TarvainenVa17} which consists of a segmentation network as student network denoted by $F^s$ and a teacher network $F^t$ with the same architecture. The weight of the teacher network $F^t$ at the $i$th iteration $\theta_i^t$ is updated as the exponential moving average of the weight $\theta_i^s$ of the student network $F^s$ given an exponential moving average decay $\eta$:
\begin{align}
\theta_i^t=\eta\theta_{i-1}^t+(1-\eta)\theta_i^s
\end{align}

Our loss function will be:
\begin{align}
\mathcal{L}=\mathcal{L}_{seg}+\mathcal{L}_{unsup}
\end{align}


%Margrit writes:  All this should be in the introduction section:
%Describe the UDA problem.\\
%Introduce current methods and their limitations.\\
%Introduce our method and its advantages, especially how it cope with the limitation and problem mentioned above.\\

We show the architecture of our model in Figure\ref{fig:overview-model}.
%Epitomize the whole process of the method briefly.

\subsection{Continuous style-guided image generator}

\input{figures/tex/alpha}

For the consideration of computational efficiency and simplicity, we adopt adaptive instance normalization~\cite{HuangBe17} to perform the image translation so that a network can learn to segment on target-domain-like images. Our continuous style-guided image generator consists of a encoder extracting a feature map from a given input image and a decoder that upsamples a feature map back to the original size of the input size. Given a content image $c$, an image that mimic the style of a style image $s$ from the other domain while pertaining its content will be synthesized. Practically, the encoder is taken from the first few layer of a pretrained fixed VGG-19~\cite{SimonyanZi15} while the decoder basically mirrors the architecture of the encoder and will be trained as in \cite{HuangBe17} before we fix and apply it in the following phases. Formally, We denotes the encoder as $f$, the decoder as $g$ and the whole generator as $T$. The feature map of a content image $c$ and a style image $s$ through the encoder $f$ could be represented as $t^c=f(c)$ and $t^s=f(s)$ such that $t^c,t^s \in \mathbb{R}^{N\times C\times H\times W}$.
% As ~\cite{HuangBe17} has shown, the style information of an image is contained in the statistics of features in a feed-forward network. Consequently, 
We can normalize the mean and the standard deviation for each channel of $t^c$ and $t^s$ and produce the target feature maps $\hat{t}$:
\begin{align}
\hat{t}={\rm AdaIN}(t^c,t^s) = \sigma(t^s)\left(\frac{t^c-\mu(t^c)}{\sigma(t^c)}\right) + \mu(t^s)
\end{align}

\[ \mu(t)=\frac{1}{HW}\sum_{h=1}^H\sum_{w=1}^W t_{nchw} \]
\[ \sigma(t)=\sqrt{\frac{1}{HW}\sum_{h=1}^H\sum_{w=1}^W(t_{nchw}-\mu(t))^2+\epsilon} \]

Once the target feature map $\hat{t}$ is obtained, we can synthesize an image from a continuous space given a content-style trade-off parameter $\alpha$ varying from 0 to 1:
\begin{align}
T(c,s,\alpha)=g(\alpha \hat{t} + (1-\alpha) t^c )
\end{align}


when $\alpha=0$, the content image will be reconstructed with its own style kept, and when $\alpha=1$, the output image will be the combination of the style of the style image $s$ and the content of the content image $c$. Finally, we rectify the output by clipping it in the range of $\left[ 0,255\right]$.

\subsection{Target-guided supervised learning}
Due to domain discrepancies between the source and target datasets, the performance of a segmentation model trained on the source dataset with pixel-level annotation will deteriorate when testing on the target domain. Nevertheless, such problem could be addressed by aligning source domain images to target domain images before a supervised loss is computed so that the segmentation model will be able to adapt better on the target domain. Given a source domain dataset $\{x_s^i, y_s^i\}$ and a target domain dataset $\{x_t^i\}$, we translate a source image $x_s$ to the style of a randomly sampled target image $x_t$ through our style-guided image generator $T$ with a content-style trade-off parameter $\alpha$ randomly sampled from an uniform distribution $\mathcal{U}(0,1)$ to get the translated image $\hat{x}_s=T(x_s,x_t,\alpha)$ with probability of $p_{s\rightarrow t}$ due to the loss of resolution in the translation process. Otherwise, we simply assign $x_s$ to $\hat{x}_s$. Finally, a cross entropy loss can be computed between the probability map $p_s=F^s(\hat{x}_s)$ and its pixel-level annotation $y_s$:

\begin{align}
\mathcal{L}_{seg}=-\frac{1}{HW}\sum_{m=1}^{H\times W}\sum_{c=1}^{C}y_s^{mc}log(p_s^{mc})
\end{align}

\subsection{Source-guided unsupervised learning}
% The scarcity of annotation in the target dataset $X^\mathcal{T}$ in UDA poses a great difficulty in adapting segmentation model on the target domain since it makes performing supervised learning impossible. Nonetheless, tremendous knowledge and information can still be exploited through semi-supervised learning without requiring those annotation. In this work, we introduce a source-guided unsupervised loss based on consistency regularization and pseudo-labeling. 

As a crucial component of consistency regularization, the stochastic image augmentation process plays a decisive role in learning from an unlabeled dataset. However, existing methods of augmentation including color space perturbation and adding Gaussian noise fail to provide satisfying performance in segmentation tasks, as observed in~\cite{FrenchAiLaMaFi2019}. They further argue that perturbations for segmentation tasks especially need to be stronger and high-dimensional so that the orientation of perturbation will be parallel to the decision boundary of a trained model rather than crossing it. Inspired by these observations, we propose a novel method to augment images that benefits the consistency regularization especially on segmentation tasks. 

To start with, we introduce the generation of the pseudo-label which guides the unsupervised learning on the target dataset. In our framework, pseudo-label will be computed from target images transferred to the direction of the appearance of the source domain where our supervised learning is performed and our model is more adapted to, so our model can generally produce pseudo-label with higher quality. Practically, we augment each target image $x_t$ using $k$ randomly sampled source images $\{x_s^i\}_{i=1}^k$ through our style-guided image generator $T$ with probability of $p_{t\rightarrow s}$ for the consideration of the loss of resolution, and $x_t$ will be transferred to a set of images $\{\hat{x}_t^i\}_{i=1}^k$ where $\hat{x}_t^i=T(x_t,x_s^i,\alpha)$. Otherwise it will only be augmented by random color space perturbations $\mathcal{A}$ to $\{\hat{x}_t^i\}_{i=1}^k=\{\mathcal{A}(x_t)\}$ with $k=1$. With the stochastic sampling of $k$ source images, our augmentation method performed on the target images will be stronger while their semantic meanings can also be preserved. After the augmentation process, transformed images $\{\hat{x}_t\}_{i=1}^k$ will be passed through the teacher model $F^t$ individually and averaged to get the probability map $p_l$ for the pseudo-label $p_l=\frac{1}{k}\sum_{i=1}^kF^t(\hat{x}_t^i)$. The reason we apply the teacher model rather than the student model is that as the temporal ensemble of the student model, the teacher model generally exhibit more stable performance to produce accurate pseudo-label. Finally we can acquire the pseudo-label $q_t$ as $q={\rm argmax}(p_l)$. 

Once the pseudo-label is computed, it can be used to guide the training of our model on the target images in a supervised manner. Concretely, we augment the same target image $x_t$ using the random color space augmentation $\mathcal{A}$ and pass it through the student network $F^s$ to get the probability map $p_t=F^s(\mathcal{A}(x_t))$. Then we can compute the unsupervised loss as follow:
\begin{align}
\mathcal{L}_{unsup}=-\frac{1}{HW}\sum_{m=1}^{H\times W}\mathbbm{1}({\rm max}(p_l^m\geq\tau))\sum_{c=1}^{C}q^{mc}log(p_t^{mc})
\end{align}
where $\tau$ is the confidence threshold which determines the assignment of pseudo-label.
\subsection{Class balancing reweight}
blablabla




% As one of the most powerful and classic semi-supervised learning approach, consistency regularization allows a model to learn from a dataset without relying on its annotation by forcing the model to produce similar predictions on a same image with different perturbations via the following loss function: 
% \begin{align}
% \mathcal{L}_{cons}=D(F(\mathcal{A}(x_m)),F(\mathcal{A}(x_m)))
% \end{align}
% where $x_m$ is an input image, $\mathcal{A}$ is a stochastic augmentation process , $F$ is a model that outputs prediction and $D$ is a distance metric. Despite the identical notation, distance between predictions will never be zero given the randomness lies in both the augmentation process $\mathcal{A}$ and the model $F$. 



% \subsection{Network Architecture}
% Image-to-image translation network: 
% Please be noted that the output image of the network will be clipped in the range of [0, 255] 


==> sections/related_work.tex <==
\section{Related Works}
% Margrit advises:
% Don't spend a lot of time on the related works until the intro is done.  In the intro, you will need to mention the limitations of existing UDA methods to explain what your contribution is.   So write that first!

%-------------------------------------------------------------------------
\subsection{Image-to-image translation}

Recent progress in image-to-image translation that transfers the style of an image while preserving its semantic content inspires various related areas, including image synthesis and merging domain discrepancy. Typical image-to-image translation approaches include CycleGAN~\cite{ZhuPaIsEf17} and DualGAN~\cite{YiZhTaGo17}, which keep cycle-consistency to preserve the semantic content of images when transferring the style of image. UNIT~\cite{LiuBrKa17} brings in an assumption of the existence of a common latent space in which a pair of corresponding images in different domains can be mapped. MUNIT~\cite{HuangLiBeKa18} further proposes that the latent space of images can be decomposed into a shared content space across all domains and an independent style space for each domain. Additionally, a noise vector is added so the image-to-image translation becomes multimodal and diverse. On the other hand, neural style transfer offers another way to perform image-to-image translation. The concept is at first proposed in~\cite{GatysEcBe16} but the optimization process is actually computationally impractical. ~\cite{JohnsonAlLi16, LiWa16,UlyanovLeVeLe16,WangOxZhWa17,UlyanovVeLe17,DumoulinShKu17,LiFaYaWaLuYa17} later improve the computation efficiency, the quality and diversity of the transferred images, but these methods are limited since the style to be transferred is either fixed or the number is limited. To address that, ~\cite{HuangBe17} proposes an arbitrary neural style transfer method that applies adaptive instance normalization on extracted features of the style and the content image.


%-------------------------------------------------------------------------
\subsection{Semi-supervised learning}

Unsupervised domain adaptation is highly related to semi-supervised learning since its target domain dataset is unlabeled. If the gap between the source and the target domain is minimized, the problem of unsupervised domain adaptation will intriguingly degenerate to semi-supervised learning and how well the information lies in the unlabeled dataset can be exploited will have a decisive effect on the performance of the method. \{As one of the most common semi-supervised learning method, pseudo-labeling, which takes predictions on the unlabeled dataset with high confidence as one-hot labels guiding further training, was used in UDA segmentation task at first by ~\cite{ZouYuKuWw18} and the concept is borrowed by other following works~\cite{LiYuVa19}\}. ~\cite{GrandvaletBe04} introduce entropy minimization into the semi-supervised learning area, which could be seen as a “soft assignment” of the pseudo-label on the unlabeled dataset. {The idea is then brought by AdvEnt~\cite{VuJaBuCoPe19} to the UDA segmentation task.} Recently, consistency regularization gains more attention and studies due to its outstanding performance as a classic yet powerful semi-supervised learning method. Mean-Teacher~\cite{TarvainenVa17} minimizes consistency loss on an unlabeled image between the output of a student network and the ensemble of itself, a teacher network. {Motivated by Mean-Teacher, ~\cite{ChoiKiKi19} exhibits encouraging performance on the UDA segmentation task}. Fixmatch~\cite{sohnBeLiZhCaCuKuZhRa20} further outperforms Mean-Teacher by performing consistency regularization and pseudo-labeling and achieves SOTA performance on several semi-supervised learning benchmarks. Concretely, the consistency loss is computed between the pseudo label produced by a segmentation model given a weakly augmented unlabeled image and its output score on the same image with another stronger augmentation. Motivated by the concept of Fixmatch combined with Mean-Teacher, we propose a novel paradigm for UDA segmentation task which guides the training of a segmentation model on a target domain image using the pseudo-label produced by its self-ensemble on the same image but in a source-like style. To the best of our knowledge, we are the first to introduce the paradigm of Fixmatch into the UDA segmentation task.

%-------------------------------------------------------------------------
\subsection{Unsupervised Domain adaptation for semantic segmentation}

Typically, an unsupervised domain adaptation segmentation method utilizes a source domain dataset with labels and a target domain dataset without labels to train a segmentation model and optimize its performance on the target domain dataset. Previous methods can be categorized into two classes: adversarial methods and non-adversarial methods. 

FCN in the wild~\cite{HoffmanWaYuDa16} is the first to perform a segmentation task under UDA settings and align both global and local features between domains through adversarial training. ~\cite{HoffmanTzPaZhIsSaEfDa18,TsaiHuScSoYaCh18,VuJaBuCoPe19} try to align features in one or multiple feature levels. In ~\cite{LuoZhGuYuYa19,WangYuWeFeXiHwHuSh20}, the adversarial alignment process of each category between domains is treated adaptively since their discrepancy might be varied. ~\cite{ChoiKiKi19} trains an image translator in an adversarial way and takes its output to perform consistency regularization. ~\cite{LiYuVa19} applies bidirectional learning that an image translator and a segmentation model guide each other’s training in a mutual way. Pseudo-labeling is also performed to enhance performance.

Other than adversarial methods, non-adversarial methods include much more diverse resorts. Curriculum DA~\cite{ZhangDaGo17} and PyCDA~\cite{LianDuLvGo19} adopt the concept of curriculum learning and align label distribution over images, landmark superpixels or regions. CBST~\cite{ZouYuKuWw18} utilize self-training to exploit information from the target domain images. DCAN~\cite{WuHaLiUzGoLiDa18} applies channel-wise alignment to merge the domain gap from both pixel-level and feature-level. Recently, Yang et al. ~\cite{YangSo20}propose to align pixel-level discrepancy by performing Fourier transformation. Combined with entropy minimization, pseudo-labeling and model ensemble, FDA achieves the current SOTA performance. 

Maybe the work most resemble ours is ~\cite{ChoiKiKi19} but our method does not rely on a strong image translator that needs to be trained in an adversarial way which might be complicated and unstable. Additionally, our method adopting consistency regularization is able to exploit information more efficiently from target images.

==> tables/augment_source.tex <==
\begin{table}[t]
  \begin{center}
  %\resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{CC|CC}
      \hline
      rAUG & S2T & mIoU & mIoU*\\
      \hline
                 &            & 33.2 & 39.5 \\
      \checkmark &            & 32.4 & 38.5 \\
                 & \checkmark & 42.0 & 48.5 \\
      \checkmark & \checkmark & \textbf{42.1} & \textbf{48.7}  \\
    \hline
    \end{tabularx}
  \end{center}
  \caption{Experiments on augmentation methods.} 
\label{tbl:augment_source}
\end{table}
